TOBUGraph: Knowledge Graph-Based Retrieval for Enhanced LLM Performance Beyond RAG

Retrieval-Augmented Generation (RAG) is one of the leading and most widely used techniques for enhancing LLM retrieval capabilities, but it still faces significant limitations in commercial use cases. RAG primarily relies on the query-chunk text-to-text similarity in the embedding space for retrieval and can fail to capture deeper semantic relationships across chunks, is highly sensitive to chunking strategies, and is prone to hallucinations. To address these challenges, we propose TOBUGraph, a graph-based retrieval framework that first constructs the knowledge graph from unstructured data dynamically and automatically. Using LLMs, TOBUGraph extracts structured knowledge and diverse relationships among data, going beyond RAG's text-to-text similarity. Retrieval is achieved through graph traversal, leveraging the extracted relationships and structures to enhance retrieval accuracy, eliminating the need for chunking configurations while reducing hallucination. We demonstrate TOBUGraph's effectiveness in TOBU, a real-world application in production for personal memory organization and retrieval. Our evaluation using real user data demonstrates that TOBUGraph outperforms multiple RAG implementations in both precision and recall, significantly improving user experience through improved retrieval accuracy.

==> 2_Tobu.tex <==
\section{TOBUGraph}

In this section, we describe TOBUGraph, a graph-based framework designed for effective information capture and retrieval, particularly in the context of personal memory organization. TOBUGraph addresses key limitations of Retrieval-Augmented Generation (RAG) approaches by dynamically extracting structured semantics and relationships from unstructured data and representing them in a graph-based structure. We implemented this approach in the TOBU app to support users in capturing and retrieving personal memories through natural and context-rich queries.

\subsection{Memory Graph Construction}

Memory construction begins when a user provides multimodal input such as images, videos, or audio recordings. A multimodal Large Language Model (LLM) processes these inputs, applying techniques such as object recognition, scene analysis, emotion detection, and geolocation inference to extract relevant contextual information. This information includes key entities such as the event date, involved individuals, locations, activities, and expressed emotions. The LLM uses these details to generate an initial textual summary of the memory.

To further refine this data, a conversational AI assistant engages with the user. It solicits additional information, clarifications, and narrative elements through a dialogue-driven interface. The memory summary is updated iteratively as users provide more input, resulting in a contextually enriched and personalized memory entry.

The structured information collected during this process is organized into a \textbf{Basic Memory Graph}. At its core, each memory is represented by a central \textbf{memory node}, which is connected to various \textbf{semantic nodes} that encode details like date, people, or place. Formally, the basic graph can be defined as \$G = (V, E)\$, where \$V = M \cup S\$ comprises the set of memory nodes \$M = {m\_1, m\_2, ..., m\_n}\$ and semantic nodes \$S = {s\_1, s\_2, ..., s\_k}\$. Edges \$E \subseteq M \times S\$ denote relationships between memory and semantic nodes. For a given memory node \$m\_i\$, its associated semantic nodes are represented as \$S\_i = { s\_j \mid (m\_i, s\_j) \in E }\$.

While the basic memory graph captures key descriptive elements of each memory, it does not yet model how different memories are conceptually or thematically connected. To address this, we introduce an augmented layer of representation: the \textbf{Relational Memory Graph (RMG)}.

\subsection{Relational Memory Graph Augmentation}

The RMG enriches the basic graph by modeling inter-memory relationships through \textbf{relationship nodes}. These nodes represent common themes or contextual anchors such as holidays, individuals, locations, preferences, or recurring activities. The system uses an LLM-based \textit{Relation Extraction Module} to analyze each memory along with its semantic context to discover patterns and shared entities across different memories.

For instance, if multiple memories refer to the theme \textit{`Halloween''}, a relationship node labeled \textit{`Halloween''} is created and connected to all relevant memory nodes. This transforms the basic graph into a richer structure \$G' = (V', E')\$, where \$V' = M \cup S \cup R\$ and \$R = { r\_1, r\_2, ..., r\_p }\$ represents relationship nodes. The edge set \$E' \subseteq (M \times S) \cup (M \times R)\$ now captures both semantic and relational linkages. Each memory node \$m\_i\$ is associated with semantic nodes \$S\_i\$ and relationship nodes \$R\_i = { r\_j \mid (m\_i, r\_j) \in E' }\$.

This graph structure enables the system to maintain a unified and connected representation of a user's memories, effectively capturing the underlying semantic and thematic relationships across diverse memory entries. The RMG thus forms the foundation for advanced, relationship-aware retrieval.

\subsection{Graph-Based Memory Retrieval}

Retrieval in TOBUGraph is performed through a conversational AI interface, allowing users to pose natural language queries about their past experiences. The system processes a user query by interacting with the RMG in three stages:

\begin{enumerate}
\item \textbf{Relationship Node Identification}: The system evaluates the query against all relationship nodes in the graph. Using prompt-based inference with an LLM, it selects a subset \$R' \subseteq R\$ of the most relevant relationship nodes that align with the query intent.
\item \textbf{Memory Traversal and Aggregation}: Once \$R'\$ is identified, the system retrieves all memory nodes \$M' \subseteq M\$ connected to \$R'\$. These memory nodes are then expanded to include their associated semantic nodes \$S' = \cup S\_i\$ for all \$m\_i \in M'\$.
\item \textbf{Response Generation}: The LLM uses the aggregated set \$M'\$ and \$S'\$ along with the original query to construct a coherent and contextually grounded response. The system is designed to provide direct answers when possible, avoiding unnecessary clarification unless the query is ambiguous.
\end{enumerate}

This process can be formalized as follows:
\begin{itemize}
\item \textbf{Relationship relevance}: \$f(q, R) \rightarrow R' \subseteq R\$
\item \textbf{Memory retrieval}: \$g(R', G') \rightarrow M' \subseteq M\$
\item \textbf{Response generation}: \$h(q, M', S') \rightarrow r\$
\end{itemize}

The graph traversal mechanism ensures that retrieval is both precise and comprehensive. Because the RMG preserves thematic connections among memories, the system can handle complex queries that involve multi-hop reasoning, pattern recognition, or semantic aggregation. For instance, it can respond effectively to prompts like, \textit{`Tell me all the trips I took with my friends in the summer,''} or \textit{`What did I do with my family during the past three Halloweens?''}

By leveraging the graph's structure, TOBUGraph eliminates the dependency on chunking strategies and reduces hallucination risk. Unlike traditional RAG systems that retrieve isolated text chunks based on embedding similarity, TOBUGraph operates on semantically grounded relationships, resulting in improved precision, recall, and user satisfaction.


==> prev_intro.tex <==
In today’s digital age, people use a variety of technologies to preserve their memories, storing images, videos, and audio to capture meaningful life moments. In 2024, an estimated 1.94 trillion photos have been taken globally, averaging 5.3 billion photos daily, with the average American capturing 20 photos per day \cite{photutorial_photos_statistics_2024}. However, to truly mimic biological memory, it is essential to capture not only the media files but also the contextual information surrounding them. Traditional media storage mechanisms fall short of preserving true `memories' as they lack the rich contextual details and narratives associated with media, such as events and sentiments. In addition, these solutions offer only limited retrieval capabilities. When retrieving a memory, users are confined to basic search and filter functionalities, making it difficult to perform natural searches like “family trips with both David and John in the mountains.”


%State-of-the-art approaches, such as those employed by social media platforms like Facebook, enable users to add basic contextual details in the form of tagging people, specifying dates and locations, and expressing feelings about the events when adding a memory input. However, these platforms provide only limited tools for memory retrieval. Users are confined to basic search and filter functionalities, making it difficult to perform nuanced searches like "family trips with both David and John in the mountains". Instead, memory retrieval often involves inefficient scrolling through chronological feeds manually or relying on simple keyword searches. Current solutions thus fall short of facilitating effortless and meaningful rediscovery of past experiences.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.75\linewidth]{TOBU app.pdf}
%     \caption{TOBU app lets users capture, store and recall digital memories, powered by conversational AI.}
%     \label{fig:tobu-app}
% \end{figure}

%TODO: might have to anonymize TOBU.

% With the rise of Large Language Models (LLMs) and their multi-modal capabilities, a possibility arises where instead of these traditional basic media storage systems, an intelligent memory storage and retrieval using LLMs.

% TOBU's mission is to address these limitations, and help users capture and preserve context-rich memories, organize them based on their relationships, just as the human brain organizes memories. In addition, TOBU aims to enable effortless and accurate memory retrieval as how humans recall relevant memories. We designed and launched a mobile application shown in Figure \ref{fig:tobu-app}, currently commercially available with a wide user base. Unlike current software solutions, TOBU presents novel capabilities to capture and retrieve memories through conversations with an AI assistant in a user-engaging manner, extracting rich context around pictures and enabling much more accurate and satisfactory memory retrieval.



%TOBU engages users through a conversational AI agent which automatically extract semantic information about memories. This approach leverages Large Language Models (LLMs) to analyze conversations and extract nuanced details

%We design and launched a mobile application TOBU is a mobile application that captures and retrieves "personal memories"(pictures/videos together with stories and context around those memories). Unlike traditional memory-capturing systems such as Apple photos or Facebook/Instagram, TOBU presents novel capabilities to capture and retrieve memories through conversations with an AI assistant through a user-engaging manner, creating and preserving the rich context and narrative around pictures.



%To address these limitations, we developed TOBU, a mobile application designed to capture and retrieve digital memories. TOBU engages users through a conversational AI agent that captures semantic information about memories. This approach leverages Large Language Models (LLMs) to analyze conversations and extract nuanced details. However, implementing an effective retrieval mechanism using conversation AI for such a memory system presented unique challenges.



% \begin{figure*}[!ht]
%     \centering
%     \begin{subfigure}[b]{0.46\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{TOBUGraph Structure.pdf}
%         \caption{}
%         \label{fig:TobuStructure}
%     \end{subfigure}
%     \hfill  % This adds horizontal spacing between subfigures
%     \begin{subfigure}[b]{0.53\textwidth}
%         \centering 
%         \includegraphics[width=\textwidth]{TOBU retrieval.pdf}
%         \caption{}
%         \label{fig:TobuRetrieval}
%     \end{subfigure}
%     \caption{TOBUGraph framework system diagram with the (a) memory capturing and (b) memory recall workflows.}
%     \label{fig:tobu_combined}
% \end{figure*}

%With the rise of Large Language Models (LLMs) and their multi-modal capabilities, digital memory storage and retrieval systems can become more effective. Instead of relying on traditional media storage and retrieval systems, these advanced approaches use LLMs to enhance memory capture and retrieval with minimal manual effort. LLMs are good at capturing context using multi-modal data \cite{wang2024comprehensivereviewmultimodallarge}. Therefore, we can apply this for capturing details related to digital memories such as time, location, and emotional significance seamlessly with less effort for the user. Also, when it comes to information retrieval from a database, we can use LLMs to context aware retrival and question and answering tasks with less effort for the user \cite{zhu2024largelanguagemodelsinformation}. It means creating a LLM driven digital memory retrieval systems can enable seamless, context-aware retrieval and filtering of memories, extending beyond basic search functions. Designing such a system involves addressing key challenges such as extracting the context and relationships about memories and enabling accurate memory retrieval. 

With the rise of Large Language Models (LLMs) and their multimodal capabilities, digital memory capturing and retrieval systems can become more effective than traditional media storage. LLMs excel at capturing context from multimodal data \cite{wang2024comprehensivereviewmultimodallarge}, allowing seamless logging of memory details such as time, location, and emotional significance. Additionally, LLMs facilitate context-aware retrieval and question-answering tasks from a given database with minimal user effort \cite{zhu2024largelanguagemodelsinformation}. This advancement paves the way for LLM-driven digital memory retrieval systems extending beyond basic search functions, offering intelligent, context-aware filtering and retrieval. However, designing such systems for effective memory capture and retrieval requires addressing key challenges, including extracting contextual relationships between memories and ensuring accurate retrieval.

In conversational AI applications, information storage and retrieval is often implemented through Retrieval-Augmented Generation (RAG) \cite{asai2023selfraglearningretrievegenerate, gao2024retrievalaugmentedgenerationlargelanguage}. RAG stores unstructured data in a vector database and retrieves it using embeddings. While RAG is effective for document-based retrieval, our initial prototype using RAG for digital memory retrieval reveals several limitations in this context.
\begin{itemize}[nosep]
    \item RAG fails to capture complex relationships between memories due to its reliance on vector embeddings.
    \item RAG's retrieval performance heavily depends on chunking and embedding strategies, often resulting in low recall or precision for memory retrieval.
    %\item Across our experiments of various embedding strategies, the low embedding quality for `memories' often leads to low precision or low recall.
    \item When related memories do not exist, LLMs may hallucinate non-existent data.
    %\item By combining chunks from various memories, it may create incorrect memories.
    %Chunks from unrelated memories can combine into incorrect or mixed results.
\end{itemize}

%or structured knowledge graph retrieval\cite{su2024knowledgegraphbasedagent, chen2024unifiedtemporalknowledgegraph}.

%TODO: need to work on this limitations together 

%To overcome these drawbacks, we can structure memories in a dynamic graph that captures relationships between them and updates automatically as new memories are added, enabling efficient graph based memory retrieval systrm. To structure data in such a manner, we can use knowledge graphs \cite{su2024knowledgegraphbasedagent}. Knowledge graphs address some of these RAG challenges by enabling fine-grained retrieval through graph traversal. However, their construction and management are labor-intensive and lack adaptability to dynamic, user-generated data.  To address this challenge, \cite{edge2025localglobalgraphrag} introduces an LLM based knowledge graph creation method. But the revival technique they are using is not relevant to our application as that technique aims to utilize in Query-focused summarization tasks.Another graph based retrieval technique is to augment LLms with graph by encouraging LLMs to reason on the graph iteratively as a chain of thought process to retrieve information (\cite{jin2024graphchainofthoughtaugmentinglarge}, \cite{Wu2024CoTKRCE}. But these two cited papers do not discuss about creating a dynamic graph as this method can only be applied when a graph is given. Therefore, although there are existing techniques to create knowledge graphs using LLms and graph based retrieval systems, there is no existing end-to-end system for graph based multi-modal information retrieval which can be applied for digital memories.   

To address these challenges of RAG, we can structure memories as a dynamic graph that captures the relationships between them, enabling an efficient graph-based memory retrieval system. A promising approach to structure data in this way is the use of knowledge graphs \cite{su2024knowledgegraphbasedagent,Hogan_2021}. Knowledge graphs addresses some of the limitations of RAG by allowing fine-grained retrieval through graph traversal \cite{barry-etal-2025-graphrag, hu2024graggraphretrievalaugmentedgeneration}. However, constructing and managing these graphs is a labor-intensive process that lacks adaptability to dynamic data \cite{Hofer_2024}. 

To overcome this challenge, \citeauthor{edge2025localglobalgraphrag} introduces an LLM-based approach to automate the creation of knowledge graphs. However, their retrieval technique primarily focuses on query-focused summarization tasks, extracting and condensing information based on a specific query. While useful for summarizing a document, this approach does not suit our application, as we need to retrieve digital memories while preserving their context and relationships. Another graph-based retrieval technique involves traversing the knowledge graph using reasoning capabilities of LLMs using a chain-of-thought process \cite{jin2024graphchainofthoughtaugmentinglarge, Wu2024CoTKRCE}. While this approach enhances retrieval capabilities, it assumes the existence of a predefined graph and does not support the creation of a dynamic knowledge graph. Thus, existing methods either enable knowledge graph creation or leverage graph-based retrieval using LLMs which can be applied to digital memories. However, they do not integrate both capture and retrieval within a single framework. %Therefore, there remains a gap where an end-to-end system does not exist for graph-based multi-modal information retrieval that can be applied for digital memories. % Filling this gap requires a novel approach that seamlessly integrates dynamic graph construction with retrieval mechanisms to organize digital memories, ensuring adaptability to evolving, user-driven data. 

Hence, we propose TOBUGraph, a novel end-to-end graph-based memory capturing and retrieval technique using LLMs. Our approach transforms multimedia files such as images, videos or audio recordings along with conversations about a memory into a structured memory graph using LLMs. The graph consists of semantic nodes representing key features of each memory, and interest nodes as common themes between various memories. These nodes are dynamically created and interlinked, enabling the system to capture nuanced relationships between memories. Unlike traditional knowledge graphs, TOBUGraph leverages LLMs for intelligent graph formation and traversal, eliminating the manual effort and facilitating comprehensive and efficient memory retrieval. By structuring memories as graph nodes, this method overcomes the limitations of RAG, improving recall and precision while minimizing hallucinations. The memory capturing technique of TOBUGraph is implemented in the real-world mobile application "TOBU," making this approach practical and usable.

%Using LLM-powered engines, these nodes are dynamically created and interconnected to establish intelligent relationships between memories, enabling comprehensive retrieval. So, this method limits incomplete or partial memory retrieval, issues when arises using a chunking method and hallucination as now this system can capture complex relatiionships that exists between memories.  As same as in traditional knowledge graphs, TOBUGraph uses graph traversal to retrieve relevant memories efficiently by leveraging nuanced relationships across different aspects of experiences but this method uses LLM in this retreival process. 
\begin{figure}[]
    \centering
    \includegraphics[width=1\linewidth]{TOBUGraph Structure.pdf}
    \caption{Memory capturing workflow in TOBUGraph framework.}
    \label{fig:TobuStructure}
\end{figure}

Using real-world data from the existing user base of the TOBU app, we evaluated the memory retrieval technique of the TOBUGraph approach against multiple RAG baseline implementations. TOBUGraph outperforms the baseline approaches in retrieval accuracy, efficiency, and user satisfaction, achieving 93.74\% $precision$ (vs. 89.23\% best baseline), 91.96\% $recall$ (vs. 82.26\% best baseline), and 92.84\% $F1$ (vs 85.56\% best baseline). It also demonstrated around 20\% improvement in user experience and satisfaction over the next-best baseline in human study, with consistently higher preference ratings in human evaluations across diverse memory recall scenarios.
%The evaluation measured the memory recall experience quantitatively through a human study and qualitatively through manual analysis of the retrieved information. TOBUGraph outperformed baseline approaches in retrieval accuracy, efficiency, and user satisfaction, achieving 92.86\% $precision$, 93.33\% $recall$, and 93.09\% $F1-score$. It also demonstrated a 14\% improvement in user experience over the next-best baseline, with consistently higher preference ratings in human evaluations across diverse memory recall scenarios. Qualitative analysis emphasized that its graph-based structure enables more accurate retrieval of relevant memories and reduces hallucination compared to other approaches.

%differing only in their memory storage and retrieval processes.
The main contributions of this paper are as follows.
\begin{enumerate} [nosep]
    \setlength{\itemsep}{0em}
    \item A novel approach to capture memories using dynamic graph structures for adaptive and context-aware retrieval, advancing beyond static knowledge representation.
    \item An LLM-powered extraction mechanism to identify and structure complex relationships between memories.
    \item  A novel graph-based memory retrieval system for enhanced user interaction.
    \item A comprehensive evaluation against RAG systems using real-world user data.
\end{enumerate}



%TOBU app is built around the TOBUGraph approach which use dynamic conversational graph-based memory capture and retrieval technique. This approach captures memories using an Large Language Models (LLM) powered conversational AI, which translates user interactions into a structured knowledge graph. The graph consists of semantic nodes, representing key features of each memory, and interest nodes, which serve as a pool of common themes between various memories. Using LLM-powered engines, these nodes are dynamically created and interconnected to establish intelligent relationships between memories.

%However, implementing such a conversational AI-powered memory retrieval system faces several technical challenges. Ensuring that LLMs provide accurate, contextually relevant details about memories while avoiding hallucinations or irrelevant outputs is critical. Additionally, managing large, dynamic memory graphs without compromising retrieval performance is technically demanding. Another hurdle is designing an interface that feels intuitive and engaging for users. The TOBUGraph approach addresses these challenges by leveraging intelligent graph-based traversal to ensure efficient and accurate memory recall. By connecting memories via interest nodes, the system reduces the need for exhaustive user input and supports more comprehensive retrieval. Also, conversational approach supports to clarify user request if it is ambiguous, allowing users to access all relevant details about their memories seamlessly as they need.



